PhyCode: A Practical Wireless Communication System Exploiting Superimposed Signals

Superimposed signals are anticipated to improve wireless spectrum efficiency to support the ever-growing IoT applications. Implementing the superimposed signal demands on ideally aligned signals in both the time and frequency domains. Prior work applied an average carrier-frequency offset compensation to the superimposed signal under the assumptions of homogeneous devices and static environments. However, this will cause a significant signal distortion in practice when heterogeneous IoT devices are involved in a dynamic environment. This paper presents PhyCode, which exploits the nature of varying offsets across devices, and designs a dynamic decoding scheme which can react to the exact offsets from different signal sources simultaneously. We implement PhyCode via a software-defined radio platform and demonstrate that PhyCode achieves a lower raw BER compared with the existing state-of-the-art method.

==> MultiHop.tex <==
%!TeX root=main.tex
\section{Relay Networks}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=6.3in]{{imag/sync_multihop}}
    \caption{Multihop Clock Alignment}
    \label{fig_sync_multihop}
\end{figure*}
Relay networks can significantly enlarge the coverage range of a transmission system, however, the disadvantage of the relay network is obvious as the throughput is limited by interference between neighbor nodes deeply. Like most of the existing works~\cite{katti2007embracing, chen2015airexpress, chen2017bipass}, mechanisms that can address the interference will directly improve the throughput. However, because these schemes transmit the analog signal among relays, every time the relay node not only amplify the information itself but also enhance the power the noise, which makes the number of the relay nodes limited by noise, 3 to 5 nodes top. Although~\cite{zhang2006hot} and its following works~\cite{lu2013implementation, you2017reliable} can denoise the signal at relay nodes to decode but they are not dedicated to multiple relays, only one rely on exists in their applications normally. Error propagation is the biggest issue, they lack the scheme that enables lower error generation and error propagation restraint. \titlename\ inspired a theoretical analysis work~\cite{zhang2017bi} that limit the error propagation problem, we further make it practical through lower error generation from a systematic point of view and eventually restraint the error propagation, which makes the relay networks promising to be implemented in existing networks. The routing protocol is not our concern in this paper, but we can build our system on top of the existing works~\cite{biswas2004opportunistic, chachulski2007trading} after the routing table is stable. To enable our scheme, we need to coordinate the transmission first, especially for the clock alignment among nodes. Next, we will detail the error propagation problem and how we solve this problem. Finally, we end up with a case study to show a real-world scenario to proof the application concept.

\subsection{Clock alignment}
As we discussed before, synchronization is the key component of our scheme. However, the synchronization among multiple relay nodes and two source nodes is quite challenging as the propagation delay cannot be easily harnessed through a compensation scheme. By doing so, we detailed our design as shown in figure~\ref{fig_sync_multihop}, where different relay nodes are separated with propagation delay $\tau_{i}$. Specifically, we can set one of the nodes as anchor node for time alignment, say starting from $t_{0}$, and all other nodes will adjust their transmitting and receiving time-based on $t_{0}$ as shown in the figure. The anchor timing node based scheme will let the system harness the challenge caused by different propagation delay, and eventually lead to a coordinated system with the aligned time source. More importantly, each node in the system only have two status, transmitting and receiving, and these two status is exchanging every time slot. Each time slot starts with the time coordinating process and ended with the last propagation completed. According to our application scenario, each time slot is around tens of microsecond, and the transmission time difference within the one-time slot is around tens of nanoseconds.

\subsection{Demodulating the signal}
Different from the analog signal based schemes, \titlename\ will repack every frame at the relay node and this process could eliminate the noise that contains in each frame. By doing so, we modulate the received signal based on the XOR principle. Although the signal can only be decoded at the sources nodes, the noise not exist anymore, and this move can reduce the noise significantly which support our system to be implemented for a larger network, such as larger monitoring system contains tens of relay nodes. Note that the modulation scheme should be consistent along all the links. More specifically, the modulation scheme is dominated by the worst channel. In particular, our scheme is focusing on the data exchanging scenarios that channel is relatively stationary.

\subsection{Stop the error propagation}

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.2in]{{imag/error_propagation_buffer}}
    \caption{Error Propagation Buffered}
    \label{fig_error_propagation}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.2in]{{imag/error_propagation_nobuffer}}
    \caption{Error Propagation No Buffer}
    \label{fig_error_propagation_nobuffer}
\end{figure}

While we design multiple schemes to harness the error sources, the bit error cannot be eliminated totally, so how to address the error propagation problem is our major challenge. Particularly, unlike traditional Wi-Fi system that each node can tell if the packet is right or wrong through CRC, our system is build upon a scheme that relay nodes can only repack the superimposed signal but can hardly tell the rightness of the signal, which means when error happens in one of the links, no one but the sources node could drop this packet. Like the related works mentioned above, the error propagation problem is always there as long as the relay nodes cannot decode the receiving packet, and this is the key feature that all these works are using to harness the neighbor interference problem. To see this problem clearly, we describe an existing procedure of the relay network that leverages the concurrent transmission to improve throughput. As we can see from figure~\ref{fig_error_propagation}, when the error happens in slot $T4$, the error package will keep bouncing around the neighboring nodes, and leads to all packets are errors at after slot $T7$.

Therefore, how to rightly sending out frames is the key method to control the error propagation problem. In doing so, \titlename\ inspired by a theoretical method that uses sources nodes to control the error~\cite{zhang2017bi}. Generally, each source node will only transmit new frames alone, instead of transmitting the linear combination of the new frame and the received frames, as shown in figure~\ref{fig_error_propagation_nobuffer}. In this way, the only disadvantage compared with existing solutions is that the source nodes need to decode the frame with higher computation complexity. But as proved in~\cite{zhang2017bi}, this complexity can easily be adopted by existing hardware. Combined with the scheme we designed before, \titlename\ can reduce the error at first place and stop the error propagation problem secondly.

==> Overview.tex <==
%!TeX root=main.tex
\section{\titlename\ Overview}
\titlename\ is a data exchanging system for the autonomous vehicle to capture other vehicles' sensing data which is NLOS or out of the detection range of data inquire vehicle. 
Inspired by existing vehicle communication system that utilizes the roadside Wi-Fi hotspot to exchange data, \titlename\ also use the Wi-Fi hotspot as transmission node but to build a relay network which can increase the vehicle's sensing range. \titlename\ is getting a much higher throughput by actively allowing the data packets to collide with other packets and can eventually decode the collision data without bringing more noise. Further, \titlename\ protects the data following in the relay links from error packet by letting the error packets itself cancel itself. To enable \titlename\ to be well implemented, following steps needed to go through:
\begin{itemize}[noitemsep,leftmargin=*]
\item \titlename\ redesign the existing Wi-Fi packet's preamble part to let it be easy detected even it collide with another packet, which follows by the redefining of the frequency offset compensation function and phase offset compensation function. 
\item \titlename\ enables higher modulation scheme after the channel estimation, a well-defined algorithm presented for relocating the constellation points according to the varying channel state of each subcarrier. 
\item \titlename\ propose an error cancellation scheme from the systematical point of view, which further lower the BER of transmitting packets.
\end{itemize}

The following sections present the details of the packet structure of \titlename\ and its transmission scheme.
